Feedback-based Modal Mutual Search for Attacking Vision-Language Pre-training Models

Although vision-language pre-training (VLP) models have achieved remarkable progress on cross-modal tasks, they remain vulnerable to adversarial attacks. Using data augmentation and cross-modal interactions to generate transferable adversarial examples on surrogate models, transfer-based black-box attacks have become the mainstream methods in attacking VLP models, as they are more practical in real-world scenarios. However, their transferability may be limited due to the differences on feature representation across different models. To this end, we propose a new attack paradigm called Feedback-based Modal Mutual Search (FMMS). FMMS introduces a novel modal mutual loss (MML), aiming to push away the matched image-text pairs while randomly drawing mismatched pairs closer in feature space, guiding the update directions of the adversarial examples. Additionally, FMMS leverages the target model feedback to iteratively refine adversarial examples, driving them into the adversarial region. To our knowledge, this is the first work to exploit target model feedback to explore multi-modality adversarial boundaries. Extensive empirical evaluations on Flickr30K and MSCOCO datasets for image-text matching tasks show that FMMS significantly outperforms the state-of-the-art baselines.

==> 07Checklist.tex <==
\newpage 
\section{Reproducibility Checklist}
This paper:
\begin{itemize}[label=\textbullet]
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)
\end{itemize}


\noindent Does this paper make theoretical contributions? (no)

% If yes, please complete the list below.

% All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
% All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
% Proofs of all novel claims are included. (yes/partial/no)
% Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
% Appropriate citations to theoretical tools used are given. (yes/partial/no)
% All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
% All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\noindent Does this paper rely on one or more datasets? (yes)
% If yes, please complete the list below.
\begin{itemize}[label=\textbullet]
    
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes)
    \item All novel datasets introduced in this paper are included in a data appendix. (no)
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (no)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (no)
\end{itemize}

\noindent Does this paper include computational experiments? (yes)
\begin{itemize}[label=\textbullet]
    
    \item Any code required for pre-processing data is included in the appendix. (yes)
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (partial)
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (no)
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
    \item This paper states the number of algorithm runs used to compute each reported result. (yes)
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (no)
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (partial)
\end{itemize}


==> Table/Symbol.tex <==
\begin{table}[!htbp]
\begin{tabular}{p{1.5cm} p{5.5cm}}
\hline
\textbf{Notation} & \textbf{Description} \\ 
\hline
$(v_{m},t_{m})$ & The matched image-text pair \\
$(v_{mis},t_{m})$ & The mismatch image and text pair \\
$(v_{m},t_{mis})$ & The image and mismatch text pair \\
$F_{I}$ & Image encoder for VLP models \\
$F_{T}$ & Text encoder for VLP models \\
$F_{I}(v)$ & Image v representation encoded by $F_{I}$ \\
$F_{T}(t)$ & Text t representation encoded by $F_{T}$ \\
$B[v,\epsilon_{v}]$ & The perturbation neighbourhood for adversarial image, where $\epsilon_{v}$ denotes the maximal perturbation bound\\
$B[t,\epsilon_{t}]$ & The perturbation neighbourhood for adversarial text, where $\epsilon_{t}$ denotes the maximal perturbation bound \\
\hline
\end{tabular}
\caption{Descriptions of each variable.}
\label{tab:notations}
\end{table}

